Properties of Galaxies and Groups: Nature versus Nurture

Due to the inherently nonlinear nature of gravity cosmological N-body simulations have become an invaluable tool when the growth of structure is being studied and modelled closer to the present epoch. Large simulations with high dynamical range have made it possible to model the formation and growth of cosmic structure with unprecedented accuracy. Moreover, galaxies, the basic building blocks of the Universe, can also be modelled in cosmological context. However, despite all the simulations and successes in recent decades, there are still many unanswered questions in the field of galaxy formation and evolution. One of the longest standing issue being the significance of the formation place and thus initial conditions to a galaxy's evolution in respect to environment, often formulated simply as "nature versus nurture" like in human development and psychology. Unfortunately, our understanding of galaxy evolution in different environments is still limited, albeit, for example, the morphology-density relation has shown that the density of the galaxy's local environment can affect its properties. Consequently, the environment should play a role in galaxy evolution, however despite the efforts, the exact role of the galaxy's local environment to its evolution remains open. This thesis introduction discusses briefly the background cosmology, cosmological N-body simulations and semi-analytical models. The second part is reserved for groups of galaxies, whether they are gravitationally bound, and what this may imply for galaxy evolution. The third part of the thesis concentrates on describing results of a case study of isolated field elliptical galaxies. The final chapter discusses another case study of luminous infra-red galaxies.

==> subfiles/abstract.tex <==
\chapter*{Abstract}\addcontentsline{toc}{chapter}{Abstract}

In this dissertation, the formation and evolution of galaxies in different
environments and formation, dynamics and structure of dark matter haloes are
studied using cosmological $N$-body simulations. The main cosmology adopted is
the standard $\Lambda$cold dark-matter (CDM) model, however, runs using different
models are used for comparison. Modeled galaxies and dark matter haloes are
compared to observed galaxies, groups and cluster of galaxies by means of
statistics.

In Paper I, we examine if cosmological simulations can produce groups of galaxies
whose properties are in agreement with observational catalogues. We also examine
if groups of galaxies are gravitationally bound structures and provide constrains
for observers that can be used to infer the probability that the group is
gravitationlly bound structure.

In Paper II, we extend our study from Paper I and provide an explanation for long
standing problem of redshift assymetries in groups of galaxies that have been
found from observed group catalogues. Gravitationally unbound groups with
misidentified centre explains the observed redshift asymmetry providing even more
support for the stardard $\Lambda$CDM cosmogony.

In Paper III, we examine if isolated field elliptical galaxies are related to
fossil groups of galaxies. We show that dark matter only cosmological $N$-body
simulations with semi-analytical galaxy formation models can form isolated
elliptical galaxies that agree with observations. However, simulations predict
previously unobserved population of blue and faint elliptical galaxies that are
yet to found.

%In Paper IV, we examine the general\ldots

==> subfiles/mypart.tex <==
\newpage
%\addcontentsline{toc}{chapter}{My contributions to the papers}

\chapter*{My contributions to the publications}

\begin{flushleft}
\begin{tabular}{ll}
\\
{\bf Are the nearby groups of galaxies gravitationally bound objects?}\\ 
Developed software to identify groups of galaxies from a cosmological $N-$body\\
simulation, conducted the analysis under supervision of Pekka Hein\"am\"aki and \\
Pasi Nurmi, and was the main writer of the publication.\\
\\
{\bf The origin of redshift asymmetries: how $\Lambda$CDM explains anomalous redshift} \\
Developed software to study redshift asymmetries, conducted the analysis under\\
supervision of Mauri Valtonen, and was the main writer of the publication.\\
\\
{\bf Formation, evolution and properties of isolated field
elliptical galaxies} \\
Developed software to identify and study isolated field elliptical galaxies,\\
conducted the analysis, and was the main writer of the publication.\\
\\
{\bf Physical properties of Herschel selected galaxies in a semi-analytical}\\ {\bf galaxy formation model}\\
Generated a mock light cone by using a semi-analytical galaxy formation model.\\
Conducted the analysis in collaboration with Rachel Somerville and Henry\\ Ferguson, and was the main writer of the publication.
\\
\\
\end{tabular}
\end{flushleft}

